Spatiotemporal Pattern Mining for Nowcasting Extreme Earthquakes in Southern California

Geoscience and seismology have utilized the most advanced technologies and equipment to monitor seismic events globally from the past few decades. With the enormous amount of data, modern GPU-powered deep learning presents a promising approach to analyze data and discover patterns. In recent years, there are plenty of successful deep learning models for picking seismic waves. However, forecasting extreme earthquakes, which can cause disasters, is still an underdeveloped topic in history. Relevant research in spatiotemporal dynamics mining and forecasting has revealed some successful predictions, a crucial topic in many scientific research fields. Most studies of them have many successful applications of using deep neural networks. In Geology and Earth science studies, earthquake prediction is one of the world's most challenging problems, about which cutting-edge deep learning technologies may help discover some valuable patterns. In this project, we propose a deep learning modeling approach, namely \tseqpre, to mine spatiotemporal patterns from data to nowcast extreme earthquakes by discovering visual dynamics in regional coarse-grained spatial grids over time. In this modeling approach, we use synthetic deep learning neural networks with domain knowledge in geoscience and seismology to exploit earthquake patterns for prediction using convolutional long short-term memory neural networks. Our experiments show a strong correlation between location prediction and magnitude prediction for earthquakes in Southern California. Ablation studies and visualization validate the effectiveness of the proposed modeling method.

==> Latex/ab-key.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
Seismology from the past few decades has utilized the most advanced technologies and equipment to monitor seismic events globally. However, forecasting disasters like earthquakes is still an underdeveloped topic from the history of mankind. Recent researches in spatial temporal forecasting have revealed some possibilities of successful predictions, which is an important topic in many scientific research fields. Most studies of them have many successful applications of using deep neural networks. In the geoscience study, earthquake prediction is one of the world's most challenging problems, about which cutting edge deep learning technologies may help to discover some useful patterns. In this project, we propose a deep learning model for earthquake forecasting. In this model, we use synthetic deep learning technologies with domain knowledge in seismology and exploit the prediction problem using convolutional long short-term memory neural networks. Our experiments show some advantages of our model in terms of location prediction and magnitude prediction for earthquakes in Southern California.
\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%
\begin{CCSXML}
<ccs2012>
 <concept>
  <concept_id>10010520.10010553.10010562</concept_id>
  <concept_desc>Computer systems organization~Embedded systems</concept_desc>
  <concept_significance>500</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010575.10010755</concept_id>
  <concept_desc>Computer systems organization~Redundancy</concept_desc>
  <concept_significance>300</concept_significance>
 </concept>
 <concept>
  <concept_id>10010520.10010553.10010554</concept_id>
  <concept_desc>Computer systems organization~Robotics</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
 <concept>
  <concept_id>10003033.10003083.10003095</concept_id>
  <concept_desc>Networks~Network reliability</concept_desc>
  <concept_significance>100</concept_significance>
 </concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Computer systems organization~Embedded systems}
\ccsdesc[300]{Computer systems organization~Redundancy}
\ccsdesc{Computer systems organization~Robotics}
\ccsdesc[100]{Networks~Network reliability}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Spatiotemporal, Convolution, LSTM, Model fusion}

==> Latex/conclusions.tex <==
\section{Conclusions and Future Work}

In this project, we discuss how we can model spatial temporal forecasting problems using deep neural networks and we propose a model to address this problem. In experiments, we demonstrate some preliminary results of using CNN-LSTM to predict earthquakes in Southern California. According our experiments, we show some promising results when proper thresholds are chosen to filter out noisy. Future works could include tuning parameters of this model and compare the performance with other models.

In future, we need to consider other physics quantities like seismicity, electric
field, magnetic field, deformation which are highly possible correlated to earthquake events.

==> Latex/exp/results.tex <==
\subsection{Discussion and Empirical Study}
We build a neural network model with CNN-LSTM layers as shown in Figure~\ref{fig:model}, in which there are 3 layers of CNN-LSTM connecting with 3 layers of Batch Normalization, and 3D convolution layer being used as the final layer.

There are two aspects in the consideration of this model:
\begin{itemize}
    \item In a period of time sequence, a sequence of $k$ 2D matrices are the input: $t_1, t_2,\ldots,t_k$, and the output is another sequence:$t_2, t_3,\ldots,t_{k+1}$. In this way, the $t_{k+1}$ is the predicted result.
    \item In Southern California, the model can be trained and predict the roughly location of the next hypocenter of earthquake with magnitude in the predicted 2D matrix. For example, if the input is $X_t$ at $t$ time, the output from the model is $X_{t+1}$ at $t+1$ time. The predicted magnitude of GEO location at $x, y$  in Southern California can be found in $X_{t+1}[y][x]$.
\end{itemize}

\subsection{Results Evaluation}

We train the model for 500 epochs. The training loss history is shown in Figure~\ref{fig:train}. The ground truth data and predicted data for 2017 and 2018 are compared in Figure~\ref{fig:pred}, in which magnitudes are normalized within range of 0 to 1 and darker cells represent higher magnitude.

\begin{equation*}
    MAPE =  \frac{100\%}{n} \frac{\sum_{i,j} \lvert \hat{y}_{i,j} - y_{i,j} \rvert }{\sum_{i,j} \lvert y_{i,j} \rvert }
\end{equation*}

To quantify the prediction, we simply calculate the coefficient of determination ($R^2$) scores between between ground truth and prediction for 2017 and 2018. Table~\ref{tbl:r2} shows the $R^2$ scores of the comparison between ground truth and prediction under different thresholds. Here the $R^2$ is defined as ${\bar {y}}={\frac {1}{n}}\sum _{i=1}^{n}y_{i}$, $SS_{\text{tot}}=\sum _{i}(y_{i}-{\bar {y}})^{2}$,$SS_{\text{reg}}=\sum _{i}(f_{i}-{\bar {y}})^{2}$, $R^{2}\equiv 1-\frac{SS_{\rm {res}}}{SS_{\rm {tot}}}$, in which $y_i$ is the ground truth and $f_i$ is the predicted data. Thresholds are used because we focus on events with big magnitudes and filter events with small magnitudes, which are tend to be just noise. According our experiments, the $R^2$ scores are 0.69, 0.71 for 2017, 2018 year respectively when the threshold is 0.25. The $R^2$ scores are 0.91, 0.93 for 2017, 2018 year respectively when the threshold is 0.3.

\begin{table}[t]
  \caption{$R^2$ score evaluation for predictions}
  \label{tbl:r2}
  \centering
  \begin{tabular}{lll}
    \toprule
    Year     & Threshold     & $R^2$ score \\
    \midrule
    2017 & 0.25  & 0.69     \\
    2017 & 0.3 & 0.91       \\
    2018 & 0.25 & 0.71      \\
    2018 & 0.3 & 0.93      \\
    \bottomrule
  \end{tabular}
\end{table}

==> Latex/experiments.tex <==
\section{Experiments and Evaluation}

\subsection{Earthquake Prediction: Dataset and Preprocessing}
The earthquake dataset is a tablet formatted dataset in which each record is an earthquake epicenter with a timestamp, a GEO location, a magnitude, and depth. In this study, we focus on the prediction of what time and location the next big earthquake will happen and the depth is ignored in this case. The dataset contains all earthquake events in Southern California ranging from 1990 to 2019 year. Figure~\ref{fig:dataset} shows all events plotted in 2D maps, in which hot spots are areas where earthquakes frequently happened or big earthquakes happened in history.

\paragraph{Data augmentation}
We divide the Southern California (Longitude: -120\textasciitilde-140, Latitude: 32\textasciitilde36) into a grid with $60\times 40$ cells, each of which has 1 degree of longitude and latitude (1 degree in kilometers is about 111km). Firstly, it is easy to group events into years. Then, let $x$, $y$ denote the longitude and latitude location of an event. All events are accumulated in corresponding cell where $x$, $y$ fall into. The value of each cell is the mean of magnitudes of all events within the cell. As a result, each year is represented by a 2D image-like matrix ($60\times 40$).

\begin{figure}
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=4cm]{Figures/mag_0.png}
        \centerline{(a) Mag $>=0$}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=4cm]{Figures/mag_2.5.png}
        \centerline{(b) Mag $>=2.5$}
    \end{minipage}
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=4cm]{Figures/mag_3.5.png}
        \centerline{(c) Mag $>=3.5$}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=4cm]{Figures/mag_4.5.png}
        \centerline{(d) Mag $>=4.5$}
    \end{minipage}
    \hfill
    \caption{Dataset}
    \label{fig:mag-list}
\end{figure}

\subsection{Experimental setup}



==> Latex/intro.tex <==
\section{Introduction}
\label{sec:intro}


Over the past few decades, large volumes of data have been collected by the seismological community. This drives high demand for seismology data processing and analysis. Spatiotemporal forecasting is an important topic in many scientific research fields, in which there are a plethora of successful applications. Recent studies using deep neural networks have shown various successful applications, including car traffic forecasting, ride-hailing forecasting, rain/weather forecasting, air pollution forecasting, etc.


\begin{figure}[hpbt]
    \begin{minipage}[b]{.48\linewidth}
      \centering
      \centerline{\includegraphics[width=4.0cm]{Figures/geo-1.png}}
    %  \vspace{1.5cm}
      \centerline{(b) Results 3}\medskip
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
      \centering
      \centerline{\includegraphics[width=4.0cm]{Figures/geo-2.png}}
    %  \vspace{1.5cm}
      \centerline{(c) Result 4}\medskip
    \end{minipage}
    %
    \caption{Dataset overview of earthquakes in Southern California.}
    \label{fig:dataset}
\end{figure}

Recent studies in deep neural networks have many successful applications of using deep learning for spatiotemporal forecasting. The goal of spatiotemporal forecasting is to predict what and when the next event will happen. This is a task that includes two orthogonal sub-tasks: forecasting its spatial dependencies and temporal dependencies. However, this is a nontrivial task due to the high dimension features of time series sequences and building models that can work well for some specific problems can also be very vague.

Earthquake forecasting is a world challenging problem. Scientists around the world have built an enormous number of detectors for picking up earthquake signals. It is a general belief that earthquakes are predictable under some assumption that quakes are formed underneath the Earth and are accumulated stresses in a gradual process for a long time. In this case, it would be possible to predict earthquake locations for future activities of quakes by learning patterns from historical seismic events.

Conventionally, earthquakes are located through a process detecting signals, picking up arrival time, and estimating epicenters of events using a velocity model. Efforts have been made to filter P-waves and S-waves from the original waveform signals of earthquakes and seismic noise. In this project, our goal is to utilize the preprocessed seismic signals forming epicenters (location labels) to forecast the locations of the next earthquakes in an area.

Earthquake forecasting locations consist of three major tasks in machine learning. The first task is to predict when the next seismic event will happen in a specific region. The second task is to predict detailed locations of the next seismic events. The third task is to predict the level of magnitude of the upcoming seismic events.

Deep learning neural networks have presented a widely successful approach to capture spatial-temporal dependencies of problems to achieve accurate forecasting results. Convolutional neural networks have achieved convinced success in computer vision, image object recognition, etc. Here we test the hypothesis that earthquakes patterns can be perceived by learning historical seismic events. However, epicenters' prediction is learned from annotated seismograms. Due to the uncertainties of earthquakes, even the ground truth labels that are annotated by domain experts may be biased. Locations and magnitude of epicenters are maybe adjusted after the seismic event happened a long while.

In this project, we propose a new self-supervised deep learning model for earthquake prediction in terms of spatiotemporal dependencies in Southern California. Our model synthetically uses convolutional neural networks and long short-term memory. Compared to conventional methods, our model presents some advantages in predicting locations and magnitude of epicenters. In summary:
\begin{itemize}
    \item We study the earthquake dataset for Southern California and reconstruct the time series events into a sequence of 2D images.
    \item We model the spatiotemporal dependencies of earthquakes in Southern California with Convolutional Long Short-Term Memory deep neural networks and show some preliminary results.
\end{itemize}



==> Latex/mm2021/ab-key.tex <==
%%
%% The abstract is a short summary of the work to be presented in the
%% article.
\begin{abstract}
    Seismology from the past few decades has utilized the most advanced technologies and equipment to monitor seismic events globally. With the enormous amount of data, modern GPU powered deep learning presents a promising approach to analyze data and discover patterns. Recent years, there are a few successful deep learning models for picking seismic waves. However, forecasting extreme earthquakes, which can cause disasters, is still an underdeveloped topic in history.  Relevant researches in spatial temporal dynamics forecasting have revealed some possibilities of successful predictions, which is an important topic in many scientific research fields. Most studies of them have many successful applications of using deep neural networks. In Geology and Earth science study, earthquake prediction is one of the world's most challenging problems, about which cutting edge deep learning technologies may help to discover some useful patterns. In this project, we propose a deep learning modeling approach to mine trajectory pattern from data for nowcasting extreme earthquakes, by discovering visual patterning in regional coarse grained spatial grids over time. In this model, we use synthetic deep learning models with domain knowledge in seismology and exploit the prediction for extreme earthquakes using convolutional long short-term memory neural networks. Our experiments show strong correlation in terms of location prediction and magnitude prediction for earthquakes in Southern California. Ablation studies and visualization validate the effectiveness of the proposed modeling method.
\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%%
\begin{CCSXML}
    <ccs2012>
    <concept>
    <concept_id>10010147.10010257.10010293</concept_id>
    <concept_desc>Computing methodologies~Machine learning approaches</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10002950.10003648.10003688.10003693</concept_id>
    <concept_desc>Mathematics of computing~Time series analysis</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    <concept>
    <concept_id>10010405.10010432</concept_id>
    <concept_desc>Applied computing~Physical sciences and engineering</concept_desc>
    <concept_significance>300</concept_significance>
    </concept>
    </ccs2012>
\end{CCSXML}

\ccsdesc[300]{Computing methodologies~Machine learning approaches}
\ccsdesc[300]{Mathematics of computing~Time series analysis}
\ccsdesc[300]{Applied computing~Physical sciences and engineering}

%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{Spatiotemporal, Convolution, LSTM, Model fusion}

==> Latex/mm2021/con-apx.tex <==
\section{Conclusions and Future Work}

In this project, we dissect the problem settings for forecasting earthquakes, discuss how we model spatial temporal forecasting problems using deep neural networks, and propose joint modeling to address this problem. In experiments, we demonstrate some preliminary results of using \tseqpre to predict earthquakes in Southern California. According our experiments, we show some promising when proper thresholds are chosen to filter out noisy. 
In future, we need to consider other physics quantities like seismicity, electric
field, magnetic field, deformation which are highly possible correlated to earthquake events.

\subsubsection*{Code and data availability}
The earthquake raw event dataset used in the paper is available to download from the USGS website at \url{https://www.usgs.gov/}. Model codes and parsed datasets used in the paper will be published upon acceptance of this manuscript.

%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
% \begin{acks}
% To Robert, for the bagels and explaining CMYK and color spaces.
% \end{acks}

==> Latex/mm2021/figures/dataset-overview.tex <==
\begin{figure}
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/mag-0.0.png}
        \centerline{(a) Mag $>=0$}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/mag-2.5.png}
        \centerline{(b) Mag $>=2.5$}
    \end{minipage}
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/mag-3.5.png}
        \centerline{(c) Mag $>=3.5$}
    \end{minipage}
    \hfill
    \begin{minipage}[b]{0.48\linewidth}
        \centering
        \includegraphics[width=\linewidth]{Figures/mag-4.5.png}
        \centerline{(d) Mag $>=4.5$}
    \end{minipage}
    % \hfill
    \Description{Dataset overview: (a) $444,589$ events with magnitude $\geq 0.0$, (b) $24,822$ events with magnitude $\geq 2.5$, (c) $2,489$ events with magnitude $\geq 3.5$, (d) $237$ events with magnitude $\geq 4.5$  }
    \caption{Dataset overview: (a) $444,589$ events with magnitude $\geq 0.0$, (b) $24,822$ events with magnitude $\geq 2.5$, (c) $2,489$ events with magnitude $\geq 3.5$, (d) $237$ events with magnitude $\geq 4.5$  }
    \label{fig:mag-list}
\end{figure}

==> Latex/mm2021/tables/ablation.tex <==
\begin{table}
    % \vspace{-0.2in}
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{3pt}
    \caption{Ablation study by removing core components in \tseqpre.}
    \label{tbl:ablation}
    % \vspace{0.1in}
    \begin{tabular}{|l|l|l|}
        \hline
        \textbf{Models}              & \textbf{F-1}    & \textbf{NSE}    \\ \hline \hline
        W/O skip connections         & 0.9001          & 0.9233          \\ \hline
        W/O local temporal attention & 0.9247          & 0.9289          \\ \hline
        \tseqpre                     & \textbf{0.9251} & \textbf{0.9323} \\ \hline
    \end{tabular}
\end{table}

==> Latex/mm2021/tables/ae-vae.tex <==
\begin{table}
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{3pt}
    \caption{\tseqpre AutoEncoder vs. VAE.}
    \label{tbl:auto-vs-vae}
    % \vspace{0.1in}
    \begin{tabular}{|l|c|c|c|}
        \hline
        \textbf{Model}                       & \textbf{MSE} & \textbf{Accuracy} & \textbf{Variance} \\ \hline \hline
        \tseqpre                             & 0.148        & 0.968             & 1.432             \\ \hline
        VAE~\cite{kingma_auto-encoding_2013} & 0.157        & 0.971             & 1.986             \\ \hline
    \end{tabular}
\end{table}

==> Latex/mm2021/tables/latent-dim.tex <==
\begin{table}
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{3pt}
    \caption{Varying the latent space dimension.}
    % \vspace{0.1in}
    \begin{tabular}{|l|l|l|}
        \hline
        \textbf{Latent space dimension} & \textbf{MSE} & \textbf{Accuracy} \\ \hline \hline
        16                              & 0.148        & 0.968             \\ \hline
        64                              & 0.140        & 0.968             \\ \hline
        128                             & 0.138        & 0.972             \\ \hline
        1024                            & 0.137        & 0.984             \\ \hline
    \end{tabular}
\end{table}

==> Latex/mm2021/tables/main-results.tex <==
\begin{table*}
    % \vspace{-0.2in}
    \centering
    % \footnotesize
    % \setlength{\tabcolsep}{3pt}
    \caption{Results comparison between \tseqpre and baseline models. Some models adopt the same architecture of using an autoencoder and a prediction network. These models are named with a `$+$' sign.\todo[inline]{Explain why some MAE are missing here so that some dumb readers can understand}}
    \label{tbl:overall}
    % \vspace{0.1in}
    \begin{tabular}{|l|r|r|r|r|r|r|}
        \hline
        \textbf{Models}   & \multicolumn{1}{l|}{\textbf{MAE}} & \multicolumn{1}{l|}{\textbf{Precision}} & \multicolumn{1}{l|}{\textbf{Recall}} & \multicolumn{1}{l|}{\textbf{F-1}} & \multicolumn{1}{l|}{\textbf{F-0.2}} & \multicolumn{1}{l|}{\textbf{NSE}} \\ \hline \hline
        MLP               & \multicolumn{1}{l|}{-}            & 0.2631                                  & 0.2845                               & 0.2096                            & 0.2494                              & -1.4739                           \\ \hline
        LSTM              & \multicolumn{1}{l|}{-}            & 0.4596                                  & 0.5186                               & 0.3801                            & 0.4058                              & -0.2059                           \\ \hline
        Conv2D-FC         & \multicolumn{1}{l|}{-}            & 0.4589                                  & 0.3963                               & 0.4340                            & 0.4394                              & -0.1867                           \\ \hline
        Conv2D-LSTM       & \multicolumn{1}{l|}{-}            & 0.4299                                  & 0.4069                               & 0.4217                            & 0.4243                              & -0.4022                           \\ \hline
        ConvLSTM2D-FC     & \multicolumn{1}{l|}{-}            & 0.4633                                  & 0.3289                               & 0.3763                            & 0.3801                              & -0.1714                           \\ \hline
        MLP+MLP           & 0.2570                            & 0.7525                                  & 0.6338                               & 0.6652                            & 0.7113                              & 0.6778                            \\ \hline
        MLP+LSTM          & 0.1637                            & 0.8420                                  & 0.7085                               & 0.7599                            & 0.8021                              & 0.7890                            \\ \hline
        MLP+Conv1D        & 0.1484                            & 0.8571                                  & 0.9351                               & 0.8029                            & 0.8342                              & 0.8133                            \\ \hline
        Conv2d+MLP        & 0.1484                            & 0.8577                                  & 0.7944                               & 0.7887                            & 0.8098                              & 0.8108                            \\ \hline
        Conv2D+LSTM       & 0.1410                            & 0.8640                                  & 0.8776                               & 0.8609                            & 0.8683                              & 0.8222                            \\ \hline
        Conv2D+Conv1D     & 0.0588                            & 0.9420                                  & 0.9115                               & 0.8998                            & 0.8688                              & 0.9293                            \\ \hline
        \textbf{\tseqpre} & \textbf{0.0483}                   & \textbf{0.9563}                         & 0.9016                               & \textbf{0.9251}                   & \textbf{0.9341}                     & \textbf{0.9323}                   \\ \hline
    \end{tabular}
\end{table*}

==> Latex/models-old.tex <==
\section{Methods: Epicenter-specific modeling}

In this section, we firstly formalize the earthquake prediction as a spatiotemporal forecasting problem in terms of its spatial and temporal dependencies. And then, we describe how the spatial and temporal dependencies can be modeled by using CNN-LSTM neural networks.

Earthquake hypocenter locations are a series of events that happened as a time sequence when different body wave phases. It is well known that these data are nonlinear functionals of the compressional or shear wave velocity structure and the coordinates of the source in space-time~\cite{Pavlis1980TheStructure.}.  Figure~\ref{fig:dataset} shows all hypocenters are plotted in maps.

% \subsection{Convolutional Neural Networks (CNN)}

% Convolutional Neural Networks (CNN) draw many successful applications in recent years and it becomes the state-of-the-art in image related approach in deep learning.
% In 2015, Berkeley~\cite{Long2015FullySegmentation} revealed that fully convolutional networks for semantic segmentation adopting AlexNet~\cite{Iandola2016SqueezeNet:Size}, VGGNet~\cite{Simonyan2014VeryRecognition}, and Google Net~\cite{Szegedy2015GoingConvolutions} can improve training and simplify the state-of-art training and inference for image classification.

% CNN has also enabled its capability to efficiently deal with spatially-correlated problems via locally-connected convolution layers.~\cite{Ji20123DRecognition}
% Geo locations of hypocenters in the earthquake dataset can be represented in graph models, in which the distance can be measured as an Euclidian distance based on longitudes and latitudes of hypocenters in 2D maps. 


% \subsection{Long Short-Term Memory (LSTM)}

% Long Short-Term Memory Neural Networks (LSTM) is a type of recurrent neural networks (RNN) in which prior knowledge can be reused~\cite{Gers1999LearningLSTM,Hochreiter1997LongMemory, Graves2013GeneratingNetworks}. LSTM is capable of learning long term dependencies by remembering information for long periods of time. We propose to use LSTM to model temporal dependence of earthquakes in time-series sequence to sequence prediction.

% \subsection{Convolutional LSTM (ConvLSTM)}

% Convolutional LSTM is an extension of fully-connected LSTM (FC-LSTM)~\cite{Shi2015ConvolutionalNowcasting}, which has convolutional LSTM and can be used to build trainable models for forecasting problems. It has been successfully adopted to predict actions affect object in a real world environment.~\cite{Finn2016UnsupervisedPrediction}
% Compare to FC-LSTM, CNN-LSTM is able to handle spatiotemporal sequences. Internally,
% spatiotemporal sequence can be transformed from a sequence of 2D matrices, which is a 3D tensor in computing.
% CNN-LSTM learns the temporal state to state transitions while keeping the spatial information via convolutions.
% The following equations show how the CNN-LSTM cell does the computation:
% \begin{equation}
%     \begin{split}
%         i_t &= \sigma(W_{xi}* X_t+W_{hi}*H_{t-1}+W_{ci} \circ C_{t-1} + b_i) \\
%         f_t &= \sigma(W_{xf}* X_t+W_{hf}*H_{t-1}+W_{cf} \circ C_{t-1} + b_f) \\
%         C_t &= f_t \circ C_{t-1} + i_t \circ tanh(W_{xc} * X_t + W_{hc} * H_{t-1} + b_c) \\
%         o_t &= \sigma(W_{xo} * X_t + W_{ho} * H_{t-1} + W_{co} \circ C_t + b_o) \\
%         H_t &= o_t \circ tanh(C_t)
%     \end{split}
% \end{equation}
% , in which $*$ represents the convolution product, $\circ$ represents the element-wise product, $X$ is the input, $C$ is the cell output, $H$ represents hidden states of cells, and $i,f,o$ are gates within cells.


\subsection{STA/LTA and Template Matching}

\subsection{Data Considerations}

The earthquake catalog is a tablet formatted dataset in which each record is an earthquake hypocenter with a timestamp, a geology location (latitude and longitude), a magnitude, and depth. In this study, we focus on the prediction of what time and location the next big earthquake will happen. The dataset contains all earthquake events in Southern California ranging from the year 1990 to 2019. Figure x shows all events plotted in 2D maps, in which hot spots are areas where earthquakes frequently happened or big earthquakes happened in history.


\paragraph{Energy-based Data Models}
Seismometers record seismic events from calibrating vibrations of waves. Magnitude in the dataset represents measured amplitude as measured seismogram [x]. While they are discrete data points, accumulating all magnitudes by summing them up by averaging makes the temporal information loss, and deemphasizes large earthquakes. In contrast to magnitude, earthquakes release energy can help mitigate this issue by two folds: 1) accumulated energy value in a region can represent the energy released by the stress of Earth over time; 2) energy data model naturally highlights large events since the energy of large events can be an order of magnitude higher than that of small events. The formula of converting earthquake magnitude to energy is defined as

\begin{equation}
    \mathbf{E} = (10^{\mathbf{M}})^{3/2}
\end{equation}
in which the magnitude $ 0 \leq \mathbf{M} \in \mathbb{R} \leq 10$. \footnote{Earthquake magnitude can be even negative for very small events that cannot felt by human. This scale is also open-ended, but events larger than 10 are extremely unlikely to happen. So these are out of the scope of this project.}

\paragraph{Location-aware data weaving} As a time-series prediction task, the earthquake catalog contains locations and magnitudes, which could be used as target properties. However, it could be more nature to reorganize the 1D time-series dataset into a 2D sequence dataset by dividing a map region into small boxes according to longitudes and latitudes and aggregating the released energy within a small box per specific time frequency. For example, we can count how much energy released within a box region of Longitude from -120 to -119 and Latitude from 32 to 33 everyday. So each element of the sequence becomes
a summation of all energy released at the location ($i,j$):    $X^t_{i,j} = \sum ((10^{\mathbf{M}})^{3/2}), i \in [0, M) $ and $j \in [0, N)$
, which means $X^t$ has a shape $M \times N$ for $M$ boxes along the latitude and $N$ boxes along the longitude.

\paragraph{Energy Value Coding}

\paragraph{Log-Energy Value Model}

\paragraph{Prediction task} This prediction task can be formalized as given a sequence of the input $ \mathbb{X} = \{X^1, X^2,\ldots,X^t\} $ that represents historical magnitudes observed from a region, learning a function $ f(\cdot) $ that maps $t$ historical signals into a future signal of magnitudes $X^{t+1}$, where $X^1,X^2,\ldots,X^t,X^{t+1} \in \mathbf{E}^{M \times N}$. This is for one-step prediction:

\begin{equation*}
    \{X_1, X_2,\ldots,X_t\} \xrightarrow{f(\cdot)} X_{t+1}
\end{equation*}
, or for multi-step prediction:
\begin{equation*}
    \{X_1, X_2,\ldots,X_t\} \xrightarrow{f(\cdot)} \{X_{t+1}, X_{t+2},\ldots,X_{t+T}\}
\end{equation*}
, in which $T$ is a hyperparameter.

\subsection{Neural Network Architecture}

\subsection{Spatial dynamics}
This neural network consists of a few residual blocks of convolutional layers with batch normalization.

\paragraph{Weighted spatial pyramid pooling} With the convolutional operations we are able to capture some general spatial structures. However, due to lack of the knowledge in the process of the earthquake deformation~[x], it is presumable unknown of how to pool local bins in convolutional operations. So, we use the weighted spatial pyramid pooling for the result of convolutions.

\paragraph{Dilated convolution} 
% DeepDetect: A Cascaded Region-Based Densely Connected Network for Seismic Event Detection
Dilated convolution essentially employs the distant information by covering large regions of input signals and maintains the same number of parameters.

\paragraph{Space structure expansion}

\subsection{Temporal dynamics}

We use a continuous-time LSTM to model temporal dynamics of earthquakes.


4.4.4	Deep Temporal Linear Encoding


4.4.7	Dropout: Normal Dropout, Spatial Dropout, and Custom Dropout
4.4.8	Feature Extractor via Transfer Learning

\subsection{Joint objective loss function}
The objective of the modeling is special to earthquake epicenters. For relative small earthquakes, we want the model can predict as precise locations as possible. Whereas, for relative large events, the location becomes less important because large hazards naturally make damages to a broad area, which means missing a large predicted event could be worse than missing lots of small ones. So the spatial precision is more sensitive for large evens than small ones. Here the $L_l$ is used to represent the location loss and $L_s$ to represent the significance loss of seismic events. In addition, $\alpha$ and $\beta$ are hyperparameters to control the importance of the location and significance.

\begin{equation}
    \begin{aligned}
    L &= \alpha L_l + \beta L_s, \\
    W_{i,j} &= \begin{cases} 1, & \mbox{if } S_{i,j} \geq threshold \\ 0, & \mbox{otherwise } \end{cases}
    \end{aligned}
\end{equation}
Here the $W$ is a mask that filters out the noisy points, which are either negligible small events or pure noise produced by the stochastic movement of earth plates [x].

==> Latex/models.tex <==
\section{TSEQPredictor}

The proposed prediction model consists of two major components, an autoencoder which learns the latent space distribution from the image like view of the earthquakes and a prediction network which learns to predict the likelihood of the next main shock happening within the same area.

\begin{figure*}[hpbt]
    \centering
    \centerline{\includegraphics[width=.88\linewidth]{Figures/TSEQNet-Predictor.pdf}}
    \caption{TSEQPredictor: overview of earthquakes in Southern California.}
    \label{fig:tseqpredictor}
\end{figure*}

\subsection{Data Considerations}
\label{sec:data-cond}

The earthquake catalog is a tablet formatted dataset in which each record is an earthquake hypocenter with a timestamp, a geology location (latitude and longitude), a magnitude, and depth. In this study, we focus on the prediction of what time and location the next big earthquake will happen. The dataset contains all earthquake events in Southern California ranging from the year 1990 to 2019. Figure x shows all events plotted in 2D maps, in which hot spots are areas where earthquakes frequently happened or big earthquakes happened in history.


\paragraph{Energy-based data models}
Seismometers record seismic events from calibrating vibrations of waves. Magnitude in the dataset represents measured amplitude as measured seismogram [x]. While they are discrete data points, accumulating all magnitudes by summing them up by averaging makes the temporal information loss, and deemphasizes large earthquakes. In contrast to magnitude, earthquakes release energy can help mitigate this issue by two folds: 1) accumulated energy value in a region can represent the energy released by the stress of Earth over time; 2) energy data model naturally highlights large events since the energy of large events can be an order of magnitude higher than that of small events. The formula of converting earthquake magnitude to energy is defined as

\begin{equation}
    \mathbf{E} = (10^{\mathbf{M}})^{3/2}
\end{equation}
in which the magnitude $ 0 \leq \mathbf{M} \in \mathbb{R} \leq 10$. \footnote{Earthquake magnitude can be even negative for very small events that cannot felt by human. This scale is also open-ended, but events larger than 10 are extremely unlikely to happen. So these are out of the scope of this project.}

\paragraph{Location-aware data weaving} As a time-series prediction task, the earthquake catalog contains locations and magnitudes, which could be used as target properties. However, it could be more nature to reorganize the 1D time-series dataset into a 2D sequence dataset by dividing a map region into small boxes according to longitudes and latitudes and aggregating the released energy within a small box per specific time frequency. For example, we can count how much energy released within a box region of Longitude from -120 to -119 and Latitude from 32 to 33 everyday. So each element of the sequence becomes
a summation of all energy released at the location ($i,j$):    $X^t_{i,j} = \sum ((10^{\mathbf{M}})^{3/2}), i \in [0, M) $ and $j \in [0, N)$
, which means $X^t$ has a shape $M \times N$ for $M$ boxes along the latitude and $N$ boxes along the longitude.

\subsection{AutoEncoder for Effective Spatial Modeling}

Main shocks with large magnitudes are rare in terms of statistics and nature physics. In addition, earthquakes are full of stochastic processing, resulting in seismic signals are very noisy. To predict the future main shocks, we first model the spatial patterns within the southern California area.

We use an autoencoder to recognize the spatial pattern changes under normal circumstances and abnormal circumstances.
This is a semi-supervised process of pretraining a model that learns the representation of earthquake images. We train this model by using the following equation.
\begin{equation}
    L(\mathbf{X_{normal}},g(f(\mathbf{X_{normal}})) + \Omega(h, \mathbf{X_{normal}})
\end{equation}
, where $ \mathbf{X_{normal}} $ are images of earthquakes with magnitudes less than a threshold, $f$ is an encoder function, $g$ is an decoder function, and $\Omega$ is a function that regularizes or penalizes the cost.

\paragraph{Spatial modeling} After the seismic events are parsed and transformed to image-like sequences in Sec~\ref{sec:data-cond}, we can utilize the spatial dependencies between pixels. Convolutional operations are common image feature extraction means. Pixel relationship can be easily mapped to geology locations of events.

\paragraph{Skip connections} We incorporate skip connections in the AutoEncoder architecture. Skip connections are forward shortcuts in networks. They symmetrically connect layers from the encoder and decoder as shown in Fig~\ref{fig:tseqpredictor}. This strategy allows long skip connections to pass features from the encoder path to the decoder path directly, which can recover spatial information lost due to downsampling, according to~\cite{he2016identity}.

\paragraph{Bottleneck layer} The bottleneck layer in the AutoEncoder is deliberately set to a small vector of a size $k$ feature map. This design is effective for two reasons. Firstly, it regularize the model to overfit all samples. Secondly, a small feature map can better differentiate the abnormal cases from normal cases.

\subsection{Predictive Model for Effective Temporal Modeling}

In this work, the goal of forecasting earthquakes is to predict the future probability of a major shock happening in Southern California. This can be done in a prediction network, which is fed in the information gained from the AutoEncoder.

\subsubsection{Conditional Temporal Convolution}

Temporal convolution neural networks are used to improve the temporal locality prediction over time. Temporal convolutional layers are layers containing causal convolution with varied dilation rate in 1D convolutional layers~\cite{oord2016wavenet,borovykh2017conditional}. A typical configuration of temporal convolution layers is set the dilation rate corresponding to the i-th of layers, for example $2^{i}$.

\begin{equation}
    p(y|\theta)=\prod_{t=0}^{T}p(y_{t+1}|y_{0},\dots,y_{t},\theta)
\end{equation}

\subsubsection{Local Temporal Attention}

A localized attention process to enhance temporal information passing is inspired by self-attention structure from Transformer~\cite{vaswani2017attention}, and Hao \etal work for sequence modeling~\cite{hao2020temporal}. The process incorporates functions $f$, $g$, and $h$ to calculate $d$ dimensional vector of keys $\mathcal{K}$, queries $\mathcal{Q}$, and values $\mathcal{V}$ respectively. Then, we calculate the weight matrix by $W=\frac{\mathcal{K}\cdot\mathcal{Q}}{\sqrt{d}}$. Finally, we apply a softmax function to the lower triangle of $W$ to get a normalized attention weight $W_{attention}=softmax(W)$ and the final out of this layer can be calculated via this attention weighted summary: $\sum_{t=0}^{T}W_{attention}\cdot y_t$.

\subsubsection{Smooth joint Nash–Sutcliffe efficiency: NSE}

NSE is widely used to evaluate predictive skills in hydrology~\cite{moriasi2007model}. NSE can
become negative when the mean error in the predictive model is larger than one standard deviation of the variability.

\begin{equation}
    NSE=1-\frac{\sum_{t=0}^{T}(\hat{y_t}-y_t)}{\sum_{t=0}^{T}(y_t-\Bar{y})}
\end{equation}

\subsection{Joint Probability Analysis}

\begin{equation}
    Loss_{AE} = MAE(\mathbf{X} - \mathbf{\Bar{X}})
\end{equation}

==> Latex/related.tex <==
\section{Related Work}

\subsection{Convolutional Methods in Predicting Epicenters}

Estimating and predicting the epicenters of earthquakes has a long history. Scientists from Geophysics, Geology and Seismology have developed a variety of tools and analytical functions to predict epicenters from datasets. In 1997, Bakun and Wentworth suggested using Modified Mercalli intensity datasets for southern California earthquakes to bound the epicenter regions and magnitudes~\cite{bakun_estimating_1997}. In 1998, Pulinets proposed predicting epicenters of strong earthquakes with the help of satellite sounding systems. Scientists from Greece had illustrated a successful project which predicted the large aspects of earthquakes using seismic electric signals~\cite{pulinets_strong_1998}. Recently, Guangmeng \etal attempted to predict earthquakes with satellite cloud images and revealed some possibilities of predicting earthquakes using geophysics data~\cite{guangmeng_three_2013}. Zakaria \etal presented their work of predicting epicenters by monitoring precursors, such as crustal deformation anomalies and thermal anomalies, with remote sensing techniques~\cite{alizadeh_zakaria_possibility_2020}. These studies either used only too little data or too simple analytical models.


\subsection{Spatiotemporal Dynamic Capture}

Most recently, it is a prevailing method to do predictions by modeling the spatial-temporal dynamics of domain science problems. This is because large volumes of data are increasingly collected in the vast majority of domains including, social science, epidemiology, transportation, and geosciences. Cui \etal proposed to use graph convolutional long short-term memory neural networks to predict traffic via capturing spatial dynamics from the car traffic patterns~\cite{cui_traffic_2019}. Li \etal utilized a seq2seq neural network architecture to capture spatial and temporal dependencies for traffic forecasting by incorporating a diffusion filter in convolutional recurrent layers~\cite{li_diffusion_2017}. FUNNEL was a project proposed by Matsubara~\cite{matsubara_funnel_2014}. It was designed to use an analytical model and a fitting algorithm for discovering spatial-temporal patterns of epidemiological data.

% \subsection{Visual Prediction Approach}
